Doubly Robust Counterfactual Classification

We study counterfactual classification as a new tool for decision-making under hypothetical (contrary to fact) scenarios. We propose a doubly-robust nonparametric estimator for a general counterfactual classifier, where we can incorporate flexible constraints by casting the classification problem as a nonlinear mathematical program involving counterfactuals. We go on to analyze the rates of convergence of the estimator and provide a closed-form expression for its asymptotic distribution. Our analysis shows that the proposed estimator is robust against nuisance model misspecification, and can attain fast $\sqrt{n}$ rates with tractable inference even when using nonparametric machine learning approaches. We study the empirical performance of our methods by simulation and apply them for recidivism risk prediction.

==> OLD/main_old.tex <==
\begin{abstract}
  The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  both the left- and right-hand margins. Use 10~point type, with a vertical
  spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  bold, and in point size 12. Two line spaces precede the abstract. The abstract
  must be limited to one paragraph.
\end{abstract}

\section{Introduction}
\label{sec:intro}


\textit{Counterfactual (or potential) outcomes} (or counterfactuals) are used to describe how a unit would respond to a specific event or treatment, irrespective of whether the event actually takes place. They are commonly used in causal inference where we would like to intervene a factual prior event and then assess the consequences of that change \citep{rubin1974estimating, holland1986statistics,hofler2005causal}. 

More recently, counterfactual outcomes have also been proved to be useful to support decision making when there is a need for predicting outcomes under hypothetical interventions. This is commonly referred to as \textit{counterfactual prediction}. Counterfactual prediction can correctly aid an important decision making in health care when randomized clinical trials are not feasible; for example, to inform decision making about treatment initiation we often require predicted risks assuming no treatment is given \citep[see, e.g.,][for more examples]{dickerman2020counterfactual, lin2021scoping}. However, the problem of counterfactual prediction brings some interesting challenges that do not arise in typical prediction problems as underlying data that we need to build predictive models are inherently not fully observable. Surprisingly, while the development of modern prediction modeling has greatly enriched causal inference via non- and semi-parametric methods \citep{kennedy2016semiparametric}, the use of causal inference to improve prediction modeling has received far less attention, although its potential is well acknowledged \citep{dickerman2020counterfactual}.

On the other hand, when building predictive models we often want to incorporate various constraints into our models. Such constraints allow us to use flexible penalization \citep{james2013penalized} or prior information \citep{gaines2018algorithms}, or to achieve fairness \citep{mishler2021fade}. In particular, we focus on the fairness constraints. By \textit{fairness}, we mean that our predictive models are not systematically biased so that the benefits (harms) do not accrue disproportionately to already (under-) privileged groups. The need of mitigating this unwanted algorithmic bias with respect to certain sensitive features (e.g., gender, race, etc.) gives rise to an unprecedented explosion of academic interest in algorithmic fairness lately \citep[see][for an overview]{barocas-hardt-narayanan}. 

In this work, we study counterfactual classification, a special case of counterfactual prediction where $Y$ is discrete, in a way that we can also minimize unfairness in models by incorporating fairness criteria. To this end, we turn our classification problem into a nonlinear constrained optimization problem where not only model accuracy but also unfairness is minimized. Then we propose an doubly robust estimator that can achieve fast root-n rates and tractable inference.



\subsection{Related Work}

Our work lies at the intersection of causal inference, algorithmic fairness, and stochastic optimization.

Counterfactual prediction is closely related to conditional average treatment effect estimation, which plays a crucial role in precision medicine and individualized policy. Let $Y^a$ denote the counterfactual outcomes that would have been observed under $A=a$, $A \in \{0,1\}$. The conditional average treatment effect (CATE) for subjects with a covariate $X=x$ is defined by $\tau(x) = \E[Y^1 - Y^0 \mid X=x]$. There exists a vast literature on estimating the CATE. There are some important early works which assumed that $\tau(x)$ follows some known parametric form \citep[e.g.,][]{van2006statistical, robins2000marginal, van2003unified, vansteelandt2014structural}. More recently, people have moved toward leveraging flexible nonparametric and machine learning methods \citep[e.g.,][]{luedtke2016super, athey2016recursive, imai2013estimating, wager2018estimation, kunzel2017meta, nie2017quasi, kennedy2020optimal, alaa2017bayesian, lu2018estimating}. A desirable property commonly held in the CATE estimation methods is that the function $\tau$ may be more structured and simple than the main effect function $\E[Y^a \mid X=x]$.

Here, we are concerned with the problem of estimating the counterfactual prediction of $\E[Y^a \mid X=x]$ under a single hypothetical intervention $A=a$, subject to fairness constraints. Without such constraints, the most straightforward approach is obtaining an identified expression for $\E[Y^a \mid X]$ and then fitting a corresponding regression or classification model. In randomized controlled trials, this is reduced to fitting a regression model $\E[Y \mid X]$ to the specific arm ($A=a$) \citep{nguyen2020counterfactual, li2016predictive}. A similar argument also applies to observational studies, which will be discussed in more detail in the next section. However, in this approach it is not clear how to incorporate the given fairness constraints into our setting, since with constraints in general our target parameter will not be given as a closed-form functional form.
% Namely, estimating $\E[Y^a \mid X=x]$ is equivalent to fitting a single regression or classification model. 

In our approach, we directly formulate and solve an optimization problem where we can flexibly incorporate fairness constraints. Most of the existing fairness literature that is concerned with observable fairness criteria. However, a growing number of recent literature have shown that counterfactuals are promising tools for algorithmic fairness. One set of fairness criteria consider counterfactuals with respect to the sensitive features
\citep{kusner2017counterfactual, nabi2018fair, nabi2019learning, wang2019equal, zhang2018fairness}. This set of counterfactual fairness criteria has brought about some controversy over whether it gives meaningful interpretation or is practically useful \citep[e.g.,][]{vanderweele2014causal}. More recently, a distinct set of approaches consider counterfactuals with respect to a decision or treatment where one can actually give an intervention \citep{mishler2021fade,mishler2021fairness, coston2020counterfactual}. Our results are closest to \cite{mishler2021fade}, who explore counterfactual fairness-accuracy tradeoffs in the regression framework based on the closed-form penalized estimators.

% Some fairness constraints do not impose restrictions on the counterfactual outcomes (e.g., the criterion of independence \citep{calders2010three}). In that case, our fairness constraints are non-counterfactual. 

More broadly, our problem can be regarded as stochastic programming in the sense that their components are unknown and thus need to be estimated. Two most common approaches in stochastic programming are {stochastic approximation} (SA) and {sample average approximation} (SAA)  \citep[e.g.,][]{nemirovski2009robust, shapiro2014lectures}. However, the standard SA and SAA approaches are not readily feasible in our setting, since we cannot compute sample moments or stochastic subgradients that involve unobserved counterfactual outcomes. Importantly, they cannot harness efficient estimators for counterfactual parameters: e.g., doubly-robust or semiparametric estimators with cross-fitting \citep[][]{Chernozhukov17, newey2018cross}. To address this issue, more general approaches beyond the SA and SAA settings may be considered \citep[e.g.,][]{dupacova1988asymptotic, shapiro1991asymptotic, shapiro1993asymptotic, shapiro2000statistical}, but these require stronger assumptions on behavior of the optimal solution and its estimator.
 

\subsection{Contribution}


\section{Problem and Setup}

Suppose that we have access to an i.i.d. sample $(Z_{1}, ... , Z_{n})$ of tuples $Z=(Y,A,S,X) \sim \Pb$ for some distribution $\Pb$, binary outcome $Y \in \{0,1\}$, pretreatment covariates $X \in \mathcal{X} \subset \R^{d_x}$, binary sensitive feature $S \in \{0,1\}$, and intervention $A \in \mathcal{A}=\{0,1\}$. For simplicity, here we assume $A$, $S$ are binary, but in principle they can be multi-valued. Let $W=(A,S,X) \in \mathcal{W}$ be the collected covariates. We are concerned with the following constrained optimization problem:
%  
\begin{equation}
\label{eqn:true-opt-problem-C}
\begin{aligned}
    & \underset{\beta \in \mathcal{B}}{\text{minimize}} \quad \mathcal{L}_{\text{CE}}\left(Y^a,\sigma(\beta, \bm{b}(W))\right) \\
    % & \text{subject to } \quad \left\vert \mathcal{U}_j(\beta,Y^a,Z;g) \right\vert \leq \delta_j \\
    & \text{subject to } \quad \left\vert \mathcal{U}_{j}(\beta,W,Y^a) \right\vert \leq \delta_j \\
    & \phantom{\text{subject to }}  \quad \,\, C\beta \leq d,
\end{aligned}     \tag{$\mathsf{P}_C$}  
\end{equation}
for some compact subset $\mathcal{B} \in \R^k$ and $C \in \R^{m\times k}$, $d \in \R^m$. 
Here, $\sigma(\cdot)$ is some $C^2$ function used to predict the score function and $\bm{b}(W)=[b_1(W),...,b_k(W)]^\top$ represents a set of basis functions for $W$ (e.g., truncated series, kernel, etc.). $\mathcal{L}_{\text{CE}}\left(Y^a,\sigma(\beta, \bm{b}(X))\right)$ is our classification risk based on the cross-entropy, and $\left\vert \mathcal{U}_{j}(\beta,W,Y^a) \right\vert$ is a magnitude of the unfairness with the $j$-th fairness criterion and corresponding tolerance level $\delta_j > 0$, each of which is defined as
\begin{align}
     \mathcal{L}_{\text{CE}}\left(Y^a,\sigma(\beta, \bm{b}(W))\right) & \coloneqq -\E\left\{ Y^a\log \sigma(\beta, \bm{b}(W)) - (1-Y^a)\log(1-\sigma(\beta, \bm{b}(W))) \right\}, \label{eqn:ce-risk} \\
     \mathcal{U}_{j}(\beta,W,Y^a)  & \coloneqq  \E\left\{g_{\text{fair},j}(W,Y^a)g_{\text{pred}}(\beta,\bm{b}(W),Y^a)\right\}, \label{eqn:unfairness-utility}
\end{align}
for some known function $g_{\text{fair},j}, g_{\text{pred}}$. We will provide more detailed explanation on $\mathcal{L}_{\text{CE}}$ and $\mathcal{U}$ shortly. 
The linear constraints $C\beta \leq d$ can be used for penalization or other practical restrictions \citep[e.g.,][]{gaines2018algorithms}. \eqref{eqn:true-opt-problem} solves our fair counterfactual classification task by minimizing both counterfactual risk and unfairness measures. We will discuss each component in further detail as follows.

\textbf{Classification risk.}
$\mathcal{L}(Y^a,\sigma(\beta, \bm{b}(W)))$ is the expected cross entropy loss for the counterfactual outcome $Y^a$ and our score function $\sigma(\beta, \bm{b}(W))$, and serves as our classification risk. Probably the most widely-used choice is the logistic regression with the given basis expansion $\bm{b}(\cdot)$, in which $\sigma(\cdot)$ is the sigmoid function that takes a single input of $\beta^\top\bm{b}(X)$ so $\mathcal{L}(Y^a,\sigma(\beta, \bm{b}(W)))$ is guaranteed to be convex. However, one may employ other more flexible classification modeling techniques such as neural networks, as long as we use a smooth, finite-dimensional parametric score function. Note that in \eqref{eqn:true-opt-problem}, we do not assume anything about the true functional relationship between $Y^a$ and $\beta$; $\beta$ is the parameter of the best-fitting function of the form $\sigma(\beta, \bm{b}(X))$.

\textbf{Unfairness Measure.}
Our unfairness measure is defined by the expected value of the two random components $g_{\text{fair}}(W,Y^a)$ and $g_{\text{pred}}(\beta,W,Y^a)$; $g_{\text{fair}}$ is a \textit{fairness function} that characterizes the nature of (un)fairness, and $g_{\text{pred}}$ is a \textit{prediction feature function} that determines which features of our predictions are to be constrained over different groups. The use of $g_{\text{fair}}$ allows us to accommodate a broad range of fairness criteria \citep[see][Section 2]{mishler2021fade}. For example, by using the following fairness functions
\begin{align*} %\label{eqn:FPR-FNR}
    g_{\text{FPR}}(W,Y^a) = \frac{(1-Y^a)(1-A)}{\E[(1-Y^a)(1-A)]} - \frac{(1-Y^a)A}{\E[(1-Y^a)A]}, \,
    g_{\text{FNR}}(W,Y^a) = \frac{Y^aA}{\E[Y^aA]} - \frac{Y^a(1-A)}{\E[Y^a(1-A)]},
\end{align*}
we can have the {false positive} and the {false negative rates} to be approximately equal across the two groups, in the sense that
\begin{align}
    & \left\vert \E\left\{g_{\text{pred}}(\beta,W,Y^a) \mid S=0, Y^a=0 \right\}  - \E\left\{g_{\text{pred}}(\beta,W,Y^a) \mid S=1, Y^a=0 \right\}\right\vert \leq \delta \label{eqn:false-positive-rate-disparity} \\
    & \left\vert \E\left\{g_{\text{pred}}(\beta,W,Y^a) \mid S=0, Y^a=1 \right\}  - \E\left\{g_{\text{pred}}(\beta,W,Y^a) \mid S=1, Y^a=1 \right\}\right\vert \leq \delta \label{eqn:false-negative-rate-disparity}.
\end{align}
This conditions require our predictions be independent of the sensitive features conditional on the counterfactual outcome $Y^a$. \eqref{eqn:false-negative-rate-disparity} alone measures violations of \textit{equal opportunity}, while \eqref{eqn:false-negative-rate-disparity} and \eqref{eqn:false-positive-rate-disparity} together measure violations of \textit{equalized odds} \citep{mishler2021fairness, hardt2016equality, barocas-hardt-narayanan}. One may use non-counterfactual fairness criteria as well. For example, by using the following fairness function
\begin{align*} 
    g_{\text{SR}}(W,Y^a) = \frac{(1-A)}{\E[1-A]} - \frac{A}{\E[A]},
\end{align*}
we can pursue the criterion of \textit{independence}:
\begin{align} \label{eqn:independence}
    \left\vert \E\left\{g_{\text{pred}}(\beta,W,Y^a) \mid S=0 \right\}  - \E\left\{g_{\text{pred}}(\beta,W,Y^a) \mid S=1 \right\}\right\vert \leq \delta,
\end{align}
which requires our predictions to be independent of the sensitive features \citep{calders2010three, barocas-hardt-narayanan}. In this case, the corresponding fairness constraints will be non-counterfactual in the sense that they do not depend on the value of $Y^a$. \\
For $g_{\text{pred}}$, one may focus on constraining the mean predictions by simply letting $g_{\text{pred}}(\beta,W)=\sigma(\beta, \bm{b}(W))$ as in most studies in the fairness literature. However in our setting, one may consider more general features of our predictions to be constrained beyond mean. For example, with some known function $g_{\text{transform}}$ one may let $g_{\text{pred}}(\beta,W)=(g_{\text{transform}}\circ \sigma)(\beta, \bm{b}(W))$ where $g_{\text{transform}}$ can be used as a weight function or to make $g_{\text{pred}}$ convex. Or we can set $g_{\text{pred},l}(\beta,W)=\left[\sigma(\beta, \bm{b}(W))\right]^l$, $l \in \mathbb{N}$ if we want to require the higher order moments, not just mean, across groups to be approximately equal. Further, if we want the classification risk itself to be approximately equal across groups, we can set $g_{\text{pred}}(\beta,W,Y^a) = \mathcal{L}_{\text{CE}}\left(Y^a,\sigma(\beta, \bm{b}(W))\right)$ $g_{\text{pred}}$. In this case, $g_{\text{pred}}$ involves the counterfactual outcome $Y^a$ as well. This shows that our framework is more general than \cite{mishler2021fade}, still being compatible with a wide collection of existing fairness criteria.


\textbf{Notation.} 
Here we give some notation used throughout this paper. For any fixed vector $v$, we let $\Vert v \Vert_2$ denote the Euclidean norm (or $L_2$-norm). $\Vert \cdot \Vert_2$ is understood as the spectral norm when it is used with a matrix. Let $\Pn$ denote the empirical measure over $(Z_1,...,Z_n)$. Given a sample operator $h$ (e.g., an estimated function), we let $\Pb$ denote the conditional expectation over a new independent observation $Z$, as in $\Pb(h)=\Pb\{h(Z)\}=\int h(z)d\Pb(z)$. Further, we use $\Vert h \Vert_{2,\Pb}$ to denote the $L_2(\Pb)$ norm of $h$ defined by $\Vert h \Vert_{2,\Pb} = \left[\Pb (h^2) \right]^{1/2} = \left[\int h(z)^2 d\Pb(z)\right]^{1/2}$. Lastly, we let $\sol(\mathsf{P})$ denote the set of optimal solutions of an optimization program $\mathsf{P}$, and define $\dist(x, S) = \inf\left\{ \Vert x - y\Vert_2: y \in S \right\}$ to denote the distance from a point $x$ to a set $S$. 

\section{Estimation Algorithm}
Let $\beta^*$ denote an optimal solution of the ``true" program \eqref{eqn:true-opt-problem} which is the parameter of interest.
Since \eqref{eqn:true-opt-problem} is not directly solvable, in order to estimate $\beta^*$ we need to find an approximating program of \eqref{eqn:true-opt-problem}. To this end, we first discuss the problem of obtaining efficient estimates for functionals of the form $\psi_a = \E\left\{\E[h_1(Y) \mid X,S,A=a ]h_2(W)\right\}$ for some known, deterministic functions $h_1:\mathcal{Y} \rightarrow \R$, $h_2:\mathcal{W} \rightarrow \R$, based on the semiparametric approach in causal inference. To simplify notation, we let  
\begin{align*}
    & \varphi_a(h_1(Y);\eta) = \frac{\mathbbm{1}(A=a)}{\pi_a(X,S)}\left\{h_1(Y)- \E[h_1(Y) \mid X,S,A]\right\} + \E[h_1(Y) \mid X,S,A=a], 
\end{align*}
denote the uncentered efficient influence functions for the parameter $\E\left\{\E[h_1(Y) \mid X,S,A=a ]\right\}$, where $\pi_a(X,S)=\Pn[A=a \mid X,S]$ is the propensity score function and $\eta=\{\pi_a(X,S), \E[h_1(Y) \mid X,S, A=a]\}$. Following \citep{}, we propose to use \textit{sample splitting} to allow for arbitrarily complex nuisance estimators $\widehat{\eta}$ and avoid empirical process conditions. Specifically, we split the data into $K$ disjoint groups by drawing variables $(B_1,..., B_n)$ independent of the data, with $B_i=b$ indicating that subject $i$ was split into group $b \in \{1,...,K\}$. Then the semiparametric estimator for $\psi_a$ based on the efficient influence function and sample splitting is given by
\begin{align} \label{eqn:semiparametric-mean-regression}
    \widehat{\psi}_a = \frac{1}{K}\sum_{b=1}^K \Pn^b\left\{\varphi_a(h_1(Y);\widehat{\eta}_{-b})h_2(W)\right\} \equiv \Pn\left\{ \varphi_a(h_1(Y);\widehat{\eta}_{-B}) h_2(W) \right\},
\end{align}
where we let $\Pn^b$ denote empirical averages only over the set of units $\{i : B_i=b\}$ in the group $b$ and let $\widehat{\eta}_{-b}$ denote the nuisance estimator constructed only using those units $\{i : B_i \neq b\}$. This semiparametric estimator attains the efficiency bound with the double robustness property, thus allows us to employ flexible machine learning methods while achieving the $\sqrt{n}$-rate of convergence and valid inference under weak conditions \citep{kennedy2016semiparametric}. % (see  and Lemma \ref{} in the appendix). 

Since each component of the program \eqref{eqn:true-opt-problem} can be represented as a smooth function of arguments of the form $\E[h_1(Y^a)h_2(W)] = \E\left\{\E[h_1(Y) \mid X,S,A=a ]h_2(W)\right\}$ for some deterministic functions $h_1, h_2$ in our setting, we can use \eqref{eqn:semiparametric-mean-regression}. With $\beta$ fixed, we estimate the classification risk as
\begin{align*}
   \widehat{\mathcal{L}}_{\text{CE}}(\beta) = -\Pn\left\{ \varphi_a(Y;\widehat{\eta}_{-B}) \log \sigma(\beta, \bm{b}(W)) - (1-\varphi_a(Y;\widehat{\eta}_{-B}))\log(1-\sigma(\beta, \bm{b}(W))) \right\}
\end{align*}
For example, if we pursue the equal opportunity in our classification with some prediction feature function $g_{\text{pred}}$ that does not involve $Y^a$, we use the estimators
\begin{align*}
   \widehat{\mathcal{U}}(\beta) = \frac{\Pn\left\{\varphi_a(Y;\widehat{\eta}_{-B})Ag_{\text{pred}}\left(\beta, b(W)\right)\right\}}{\Pn\left\{\varphi_a(Y;\widehat{\eta}_{-B})A\right\}} - \frac{\Pn\left\{\varphi_a(Y;\widehat{\eta}_{-B})(1-A)\left(\beta, b(W)\right)\right\}}{\Pn\left\{\varphi_a(Y;\widehat{\eta}_{-B})(1-A)\right\}},
\end{align*}
for $\mathcal{L}_{\text{CE}}\left(Y^a,\sigma(\beta, \bm{b}(W))\right)$ and $\E\left\{g_{\text{FNR}}(W,Y^a)g_{\text{pred}}(\beta,W)\right\}$, respectively, where $\eta=\{\pi_a(X,S), \E[Y \mid X,S, A=a]\}$. In Appendix \ref{}, we enumerate our proposed estimators for other choices for $g_{\text{fair}}$ and $g_{\text{pred}}$ as well.

Now that we have proposed the efficient methods to estimate each component of the true program \ref{eqn:true-opt-problem}, we give an approximating program that we aim to solve to estimate $\beta^*$. The most straightforward way is to estimate $\widehat{\mathcal{L}}_{\text{CE}}$ and $\widehat{\mathcal{U}}_j's$, and then plug back into the original program \ref{eqn:true-opt-problem-C}. Next, when all the $\widehat{\mathcal{U}}_j's$ are convex, we can instead aim to solve the following unfairness penalized (Lagrange) form for some $\lambda_j>0$:
\begin{equation}
\label{eqn:true-opt-problem-L}
\begin{aligned}
    & \underset{\beta \in \mathcal{B}}{\text{minimize}} \quad \mathcal{L}_{\text{CE}}\left(Y^a,\sigma(\beta, \bm{b}(W))\right) + \sum_j \lambda_j\left\{ \mathcal{U}_{j}(\beta,W,Y^a) \right\}^2 \\
    & \text{subject to } \quad C\beta \leq d.
\end{aligned}     \tag{$\mathsf{P}_L$}  
\end{equation}

\begin{claim}
Let $\beta^*$ denote an optimal solution in \ref{eqn:true-opt-problem-L} for some $\lambda_j>0$. If each $\widehat{\mathcal{U}}_j$ is convex, then $\beta^*$ is also an optimal solution in \ref{eqn:true-opt-problem-C} with $\delta_j^2 = \left(\E\left\{g_{\text{fair},j}(W,Y^a)g_{\text{pred}}(\beta^*,\bm{b}(W),Y^a)\right\}\right)^2$. If we further assume the Linear Independence Constraint Qualification (LICQ) for \ref{eqn:true-opt-problem-C}, then \ref{eqn:true-opt-problem-C} and \ref{eqn:true-opt-problem-L} are equivalent.
\end{claim}

Consequently, we consider the following two approximating programs \ref{eqn:approx-C} and \ref{eqn:approx-L}, and aim to compute their optimal solutions $\widehat{\beta}$ as our estimate for $\beta^*$.

\begin{minipage}{.4\textwidth}
\begin{equation}
\label{eqn:approx-C}
    \begin{aligned}
        &\underset{\beta \in \mathcal{B}}{\text{minimize}} \quad \widehat{\mathcal{L}}_{\text{CE}}(\beta) \\
        &\text{subject to} \,\, \begin{cases}\left\vert \widehat{\mathcal{U}}_j(\beta) \right\vert \leq \delta_j\\ C\beta \leq d\end{cases} 
    \end{aligned} \tag{$\widehat{\mathsf{P}}_C$}  
\end{equation} 
\end{minipage}%
\hfill
\begin{minipage}{.5\textwidth}
\begin{equation}
\label{eqn:approx-L}
    \begin{aligned}
        & \underset{\beta \in \mathcal{B}}{\text{minimize}} \quad \widehat{\mathcal{L}}_{\text{CE}}(\beta) + \sum_j \lambda_j\left\{ \widehat{\mathcal{U}}_{j}(\beta) \right\}^2 \\
        & \text{subject to} \quad C\beta \leq d
    \end{aligned} \tag{$\widehat{\mathsf{P}}_L$}  
\end{equation}
\end{minipage}

Although it seemed that \ref{eqn:approx-C} is the most natural way to estimate $\beta^*$, it requires very strong assumptions to establish consistency of our estimator $\widehat{\beta}$ due to its stochastic feasible set. On the other hand, \ref{eqn:approx-L} requires the convexity of $\widehat{\mathcal{U}}_j$ and only allows the indirect control over unfairness via penalization, but we can enjoy much weaker assumptions to achieve the fast rates of convergence for $\widehat{\beta}$. This will be discussed in more details in the following section.

% In the following section, we will discuss in more details conditions to describe the asymptotic behavior of $\widehat{\beta}$ in both \ref{eqn:approx-C} and \ref{eqn:approx-L}.


\section{Asymptotic Analysis}




For some $h_y: \mathcal{Y} \rightarrow \R$, let $\mu_{a}=\E[h_y(Y) \mid X,S, A=a]$, so $\eta=\{\pi_a, \mu_{a}\}$. Assume the following:

\begin{enumerate}[label={}, leftmargin=*]
	    \item \customlabel{assumption:A1}{(A1)} either i) $\widehat{\eta}$ are estimated using sample splitting or ii) the function class  $\{\varphi_a(\cdot;\eta): \eta \in (0,1)^2\times \R^2\}$ is Donsker in $\eta$
	    \item \customlabel{assumption:A2}{(A2)}  $\Pb(\widehat{\pi}_a \in [\epsilon, 1-\epsilon]) = 1$ for some $\epsilon > 0$ 
	    \item \customlabel{assumption:A3}{(A3)} $\Vert \widehat{\mu}_{a}- \mu_{a} \Vert_{2,\Pb} = o_\Pb(1)$,
	    \item \customlabel{assumption:A4}{(A4)}  
	    $   \begin{aligned}[t]
            &\Vert \widehat{\pi}_{a} - {\pi}_{a} \Vert_{2,\Pb} \Vert \widehat{\mu}_{a} - \mu_{a} \Vert_{2,\Pb} = o_\Pb(n^{-1/2}), 
            \end{aligned} 
        $
\end{enumerate}	  

Assumptions \ref{assumption:A1} - \ref{assumption:A4} are commonly used in the semiparametric literature \citep{}. 

\begin{theorem}[Rate of Convergence] \label{thm:convergence-rates}
Provided that $\widehat{\mathcal{U}}_j$ is a convex function of class $C^2$, let $\widehat{\beta}_L$ denote an optimal solution in \ref{eqn:approx-L}. If we assume \ref{assumption:A1} - \ref{assumption:A3}, then
\begin{align*}
    \dist\left(\widehat{\beta}_L , \sol(\text{\ref{eqn:true-opt-problem-L}})\right) &= O_\Pb\left(\Vert \widehat{\pi}_a - \pi_a \Vert_{2,\Pb} \Vert \widehat{\mu}_{a}- \mu_{a} \Vert_{2,\Pb} \right).
\end{align*}
If we further assume the nonparametric condition \ref{assumption:A4}, then we obtain
\begin{align*}
    \dist\left(\widehat{\beta}_L , \sol(\text{\ref{eqn:true-opt-problem-L}})\right) &= O_\Pb\left(n^{-1/2} \right).
\end{align*}
\end{theorem} 

Note that other than the smoothness and convexity of $\widehat{\mathcal{U}}_j$, we do not require any regularity conditions (neither deterministic nor stochastic) on \ref{eqn:true-opt-problem-L} to derive the rate of convergence of $\widehat{\beta}_L$. This is generally not true in stochastic programming.

\begin{theorem}[Asymptotic Distribution] \label{thm:asymptotics}
Assume the same conditions of Theorem \ref{thm:convergence-rates}.
Further assume that


\end{theorem} 

\section{Simulation and Case Study}
\subsection{Simulation}
We first explore the finite sample properties of our estimators in the simulated dataset.

The data generating process is as follows

\subsection{Case Study: COMPAS Dataset}
Next we apply our method in recidivism risk prediction using the COMPAS dataset \citep{}. This dataset comprises

\section{Discussion}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Our work focuses on the methodological development and is not tied to particular applications. Also, our methods do not suggest any particular ways to quantify fairness. Hence discussion about potential negative societal impacts is not applicable to ours.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec:asymptotics}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Section \ref{appendix:proof} in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{We have only used the public data and the open-source packages in R (see Section \ref{sec:experiments}).}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
